Universalizing Weak Supervision

Weak supervision (WS) frameworks are a popular way to bypass hand-labeling large datasets for training data-hungry models. These approaches synthesize multiple noisy but cheaply-acquired estimates of labels into a set of high-quality pseudolabels for downstream training. However, the synthesis technique is specific to a particular kind of label, such as binary labels or sequences, and each new label type requires manually designing a new synthesis algorithm. Instead, we propose a universal technique that enables weak supervision over any label type while still offering desirable properties, including practical flexibility, computational efficiency, and theoretical guarantees. We apply this technique to important problems previously not tackled by WS frameworks including learning to rank, regression, and learning in hyperbolic space. Theoretically, our synthesis approach produces a consistent estimators for learning some challenging but important generalizations of the exponential family model. Experimentally, we validate our framework and show improvement over baselines in diverse settings including real-world learning-to-rank and regression problems along with learning on hyperbolic manifolds.

==> macros.tex <==
\newcommand{\yell}[1]{\textcolor{red}{#1}}
% \newcommand{\assume}[1]{\textcolor{blue}{\textbf{#1}}}
\newcommand{\assume}[1]{#1}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{observation}{Observation}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}

%% OPERATORS:
\newcommand{\norm}[1]{\left|\left|#1\right|\right|}
\newcommand{\argmin}[2]{\textrm{argmin}_{#1}~#2}
\newcommand{\argmax}[2]{\textrm{argmax}_{#1}~#2}
% Inner product
\newcommand{\ip}[2]{\left\langle#1, #2\right\rangle}
% Trace
\newcommand{\tr}{\textrm{tr}}
% Expected value
\newcommand{\E}[2]{\mathbb{E}_{#1}\left[#2\right]}
% Sample mean
\newcommand{\Ehat}[1]{\hat{\mathbb{E}}\left[#1\right]}
% Variance
\newcommand{\Var}[2]{\textrm{Var}_{#1}\left[#2\right]}
% Covariance
\newcommand{\Cov}[2]{\textrm{\textbf{Cov}}_{#1}\left[#2\right]}
% Indicator
\newcommand{\ind}[1]{\mathbbm{1}\left\{#1\right\}}
\newcommand{\indpm}[1]{\mathbbm{1}^{\pm}\left\{#1\right\}}
% sech
\newcommand{\sech}[0]{\textrm{sech}}
% diag
\newcommand{\diagm}[1]{\textrm{diagm}\left(#1\right)}
% supp
\newcommand{\supp}{\text{supp}}
% independent
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

%\newenvironment{bsmallmatrix}
%  {\left[\begin{smallmatrix}}
%  {\end{smallmatrix}\right]}


%% VARIABLES:
% See Glossary of Symbols (Appendix A.1)
\newcommand{\x}[0]{X}
\newcommand{\p}[0]{\mathcal{P}}
\newcommand{\y}[0]{Y}
\newcommand{\lf}[0]{\lambda}
\newcommand{\lfc}[0]{\Lambda}
\newcommand{\acc}[0]{\alpha}



% LF outputs
\newcommand{\lx}[0]{\lambda}
% Observed LF outputs
\newcommand{\lfo}[0]{\bar{\lf}}
\newcommand{\lxo}[0]{\bar{\lx}}

% see line at top of main file to show/hide notes
\ifdefined\ShowNotes
  \newcommand{\colornote}[3]{{\color{#1}\bf{#2 #3}\normalfont}}
\else
  \newcommand{\colornote}[3]{}
\fi

\definecolor{darkred}{rgb}{0.7,0.1,0.1}
\definecolor{darkgreen}{rgb}{0.1,0.5,0.1}
\definecolor{cyan}{rgb}{0.7,0.0,0.7}
\definecolor{dblue}{rgb}{0.2,0.2,0.8}
\definecolor{maroon}{rgb}{0.76,.13,.28}
\definecolor{burntorange}{rgb}{0.81,.33,0}
\definecolor{royalpurple}{rgb}{0.47,.31,0.66}

% \newcommand {\note}[1]{\colornote{maroon}{}{#1}}
\newcommand {\todo}[1]{\colornote{cyan}{TODO}{#1}}
\newcommand {\dan}[1]{\colornote{darkgreen}{DF:}{#1}}
\newcommand {\fred}[1]{\colornote{burntorange}{FS:}{#1}}
\newcommand {\mayee}[1]{\colornote{red}{MC:}{#1}}

% not a colornote since we don't want these to ever be removed from the document
\ifdefined\ShowNotes
  \newcommand{\num}[1]{{\color{red}\bf{#1}\normalfont}}
\else
  \newcommand{\num}[1]{#1}
\fi

\newcommand{\sysx}{\textsc{FlyingSquid}}
\newcommand{\avgspeedupdugong}{\num{2,300}}
\newcommand{\maxspeedupdugong}{\num{4,000}}
\newcommand{\avgspeedupdp}{\num{235}}
\newcommand{\maxspeedupdp}{\num{348}}
\newcommand{\avgspeedupdpbench}{\num{170}}
\newcommand{\maxspeedupdpbench}{\num{440}}
\newcommand{\avgspeedupdpbenchround}{\num{170}}
\newcommand{\maxspeedupdpbenchround}{\num{440}}
\newcommand{\avgslowdowndugongdp}{\num{9.5}}

\newcommand{\avglifttsall}{\num{13.4}}
\newcommand{\maxlifttsall}{\num{29.3}}
\newcommand{\avgliftmvall}{\num{14.7}}
\newcommand{\maxliftmvall}{\num{33.9}}
\newcommand{\avgliftts}{\num{12.4}}
\newcommand{\maxliftts}{\num{25.2}}
\newcommand{\avgliftmv}{\num{16.7}}
\newcommand{\maxliftmv}{\num{33.9}}
\newcommand{\avgliftdp}{\num{28.9}}
\newcommand{\maxliftdp}{\num{83.2}}
\newcommand{\avgliftdugong}{\num{1.1}}
\newcommand{\maxliftdugong}{\num{2.5}}
\newcommand{\avgliftdpbench}{\num{2.3}}
\newcommand{\maxliftdpbench}{\num{4.9}}
\newcommand{\avglifttsonline}{\num{19.8}}
\newcommand{\maxlifttsonline}{\num{36.5}}
\newcommand{\avgliftmvonline}{\num{8.9}}
\newcommand{\maxliftmvonline}{\num{15.7}}
\newcommand{\avgliftrandomabstains}{\num{25.6}}
\newcommand{\maxliftbestsingletriplet}{\num{4.2}}
\newcommand{\avgliftsingletriplet}{\num{23.8}}

\newcommand{\spam}{\textbf{Spam}}
\newcommand{\spouse}{\textbf{Spouse}}
\newcommand{\weather}{\textbf{Weather}}
\newcommand{\recommender}{\textbf{Recommender}}
\newcommand{\interview}{\textbf{Interview}}
\newcommand{\commercial}{\textbf{Commercial}}
\newcommand{\tennis}{\textbf{Tennis Rally}}
\newcommand{\basketball}{\textbf{Basketball}}
% \newcommand{\shot}{\textbf{Shot Detection}}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
% \newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
% \newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes
  \item Did you describe the limitations of your work?
    \answerYes
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section \ref{sec:theory} and Appendix}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See Section \ref{sec:theory} and Appendix}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We include them in supplemental materials.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section \ref{sec:experiment} and Appendix.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Section \ref{sec:experiment} and Appendix.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section \ref{sec:experiment} and Appendix}
  \item Did you mention the license of the assets?
    \answerNA{The license of datasets are described in provided URLs.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See References}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{Datasets were collected through official APIs.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{Datasets don't include information about individuals.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> sections/known_results.tex <==
\section{Known Results}
\subsection{Full Ranking}
\subsubsection{Single Parameter }
Its the basic setup where Mallows' distribution is parameterized by a single spread parameter $\phi \in [0,1]$ and central ranking $\pi^* \in S_d$. Here we observe $n$ i.i.d samples $\pi \in S_d$

\begin{theorem} \cite{caragiannis2016}
	For any given $\epsilon > 0$, any PM-c rule determines the true ranking with probability at least $1-\epsilon$ given  $\mathcal{O}(\log(\frac{d}{\epsilon}))$  samples from Mallows' model.
\end{theorem}

\begin{theorem}
	\cite{optimalMallows2019} For any given $\pi^* \in S_d$ and $\phi^* \in [0,1-\gamma]$ Then there exist estimates $\hat{\phi}, \hat{\pi}$ which can be computed in polynomial time using $n \ge \Omega \Big( \frac{\log(1/\delta)}{d\epsilon^2} + \frac{1}{\gamma} \log(d/\delta)\Big)$ such that \begin{equation} Pr\big( (\pi^*=\hat{\pi}) \land (|\phi^*-\hat{\phi}|\le \epsilon) \big ) \ge 1-\delta.
	\end{equation}
\end{theorem}


\textbf{RQ1} One might need samples lower than $\log(d/\epsilon)$ if the goal is to find $\hat{\pi}$ such that $d_\tau(\hat{\pi},\pi^*) \le \kappa$ 
\subsubsection{Generalized Mallows}
\cite{optimalMallows2019}

\subsection{Partial Ranking}
\subsubsection{Single Parameter}
In this setup we observe partial rankings of length $k$ over $d$ objects ($k\le d$). The The definition of Mallows' distribution is changed a bit in this case. Here $\pi^*$ is a partial ranking of length $k$ and the Kendall's Tau distance is also adapted accordingly as following, 
\begin{equation}
	d'_\tau(r1,r2) = \sum_{i,j \in r1\cup r2 \; i<j} X_{ij}
\end{equation}
\begin{equation} 
	X_{ij} = 
	\begin{cases}
		& 1 \quad \text{if } (i <_{r_1} j \text{ and } i >_{r2} j) \text{ or vice versa}  \\
		& p \quad \text{if } (i \perp_{r_1} j \text{ and } i \parallel_{r2} j) \text{ or vice versa} \\
		&  0  \quad \text{otherwise}
	\end{cases}
\end{equation}

\begin{theorem} \cite{flavioTopK2018}
	There exists a polynomial time algorithm that uses $\Theta \Big ( \frac{\phi +1}{\phi^{-1} -1} (d-k) \log d\Big  ) $ i.i.d. samples from the Mallows' distribution and can identify the central top-k list with probability $1 - o(n^{-3})$
\end{theorem}

\cite{fotakis21Selective}
\subsubsection{Generalized Mallows'}

\begin{section}{Weak Supervision with Rankings}
	\begin{itemize}
		\item Samples are from different $\phi$ but same center. We want to aggregate them to find the center. How similar is it to mixture model? Is it special case of mixture model where centers are same. Assume that $\phi$ are given, then derive sample complexity bounds to recover the center. 
		
		\item Samples are from different centers and we want to estimate $\phi$.
		
		\item Do both of the above for partial / top-k lists settings.
		
		\item Do all the above with generalized Mallows'. 
		
	\end{itemize}
\end{section}



==> sections/learning_acc.tex <==
\section{Learning accuracies of LFs in Ranking setup}
Let there be $d$ items over which $m$ LFs, give their orderings. Denote true ranking by $Y$ and ranking by $i^{th}$ LF as $\pi_i$. Let the items be indexed from $1$ to $d$ and define $S=\{(i,j): i < j ; i,j\in[d]\}$ and $S$ is ordered by $i$. In order to capture agreement and disagreement between any two rankings $r_1$ and $r_2$ we define  $\mathbf{Z}(r_1,r_2) \in \{-1,+1\}^{|
	S|}$ as following, 
\begin{equation}
	\mathbf{Z}(r_1,r_2)_i &=
	\begin{cases}
		+1 & \text{ if } r_1, r_2 \text{ agree on } i^{th} \text{ pair} \\  
		-1 & \text{ if } r_1, r_2 \text{ disagree on } i^{th} \text{ pair}
	\end{cases}
\end{equation}
Kendall Tau correlation coefficient between two rankings $r_1, r_2$ can be written as,
\begin{equation}
	d_\tau(r_1,r_2) = \frac{1}{|S|}\sum_i \mathbf{Z}(r_1,r_2)_i
\end{equation}
We want to estimate  $\mathbb{E}[ d_\tau(Y,\pi_k)]$ = $\frac{1}{|S|}\sum_{i} \mathbb{E}[ \mathbf{Z}(Y,\pi_k)_i]$ as a proxy for accuracy of $k^{th}$ LF.
Define $\mathbf{Z}^{(k)} = \mathbb{E}_{Y,\pi_k}[ \mathbf{Z}(Y,\pi_k)] \in \mathbb{R}^{|S|}$. We want to learn $\mathbf{Z}^{(k)}$ but we neither have access to the true distribution nor do we have access to samples of $Y$ so we can't even do an empirical estimation.

Observe that for any two LFs, $k,\ell$, we have  $\mathbf{Z}^{(k)}_i \cdot \mathbf{Z}^{(\ell)}_i = \mathbb{E}_{Y,\pi_k,\pi_{\ell}}[\mathbf{Z}(Y,\pi_k)_i \cdot \mathbf{Z}(Y,\pi_{\ell})_i] = \mathbb{E}_{\pi_k,\pi_{\ell}}[\mathbf{Z}(\pi_k,\pi_\ell)_i]$ . 
This holds $\mathbf{Z}(Y,\pi_k)_i \cdot \mathbf{Z}(Y,\pi_{\ell})_i = +1$ when both $\pi_k, \pi_{\ell}$ agree or disagree with $Y$ and it is equal to -1 when only one of them agrees with $Y$, which is equivalent to measuring their own agreement and disagreements.
We can have an empirical estimate $\hat{\mu}_{k,\ell}^{(i)}$ of $\mathbb{E}_{\pi_k,\pi_{\ell}}[\mathbf{Z}(\pi_k,\pi_\ell)_i]$ using which we can get empirical estimate $\hat{\mathbf{Z}}^{(j)}$ of accuracies for all LFs. 

Lets consider a simple example with three LFs. For $i^{th}$ pair,
\begin{equation}
	\begin{split}
		\hat{\mathbf{Z}}^{(1)}_i \cdot \hat{\mathbf{Z}}^{(2)}_i &=  \hat{\mu}_{1,2}^{(i)}   \\
		\hat{\mathbf{Z}}^{(2)}_i \cdot \hat{\mathbf{Z}}^{(3)}_i &=  \hat{\mu}_{2,3}^{(i)}   \\
		\hat{\mathbf{Z}}^{(1)}_i \cdot \hat{\mathbf{Z}}^{(3)}_i &=  \hat{\mu}_{1,3}^{(i)}   
	\end{split}
\end{equation}
solving this system of equation yields,
\begin{equation}
	\begin{split}
		\hat{\mathbf{Z}}^{(1)}_i &= \sqrt{\hat{\mu}_{1,2}^{(i)}\hat{\mu}_{1,3}^{(i)}/\hat{\mu}_{2,3}^{(i)}} \\
		\hat{\mathbf{Z}}^{(2)}_i &= \sqrt{\hat{\mu}_{1,2}^{(i)}\hat{\mu}_{2,3}^{(i)}/\hat{\mu}_{1,3}^{(i)}} \\
		\hat{\mathbf{Z}}^{(3)}_i &= \sqrt{\hat{\mu}_{1,3}^{(i)}\hat{\mu}_{2,3}^{(i)}/\hat{\mu}_{1,2}^{(i)}}
	\end{split}
\end{equation}
We do it for all pairs $i$ and finally get estimated accuracy of $k^{th}$ LF,  $\hat{\mathbf{Z}}^{(k)} = \frac{1}{|S|} \sum_i \hat{\mathbf{Z}}^{(k)}_i  $

\subsection{Analysis of Synthetic Setup}
Let's denote a ranking by its agreement/disagreement to a reference ranking so that each ranking belongs to $\{-1,+1\}^{|S|}$. Let $\alpha_i,\beta_i \in [0,1] $ be accuracy parameters of $i^{th}$ LF. Assume the labeling functions produce ranking by following this process:
\begin{enumerate}
	\item For given ranking $Y$, the $i^{th}$ LF will first decide whether or not make any change in $Y$ with probability $1-\alpha_i$. Denote this decision variable by $z \in \{0,1\}$, where $z=1$ indicates $Y$ will be perturbed. 
	\item If in the previous step $z=1$ then each pair in $Y$ will be inverted with probability $1-\beta_i$.
\end{enumerate}
The inner product $\langle Y,\pi_i \rangle$ tells how well do $Y,\pi_i$ agree and $\frac{1}{|S|}\langle Y,\pi_i \rangle $ is precisely the Kendall's-tau correlation coefficient between the two.
We are interested in computing $\mathbb{E}[\langle Y,\pi_i\rangle]$ which will give us the expected Kendall's tau correlation between rankings produced by LF $i$ and true rankings.
\paragraph{Binary Case}:\\

Here we have only two items i.e. a single pair hence $Y,\pi_i \in\{+1,-1\}$. In this setup $\beta_i$ doesn't make sense so we assume it be 0.
\begin{equation}
	\mathbb{E}[Y\pi_i] = (1)\alpha_i + (-1)(1-\alpha_i) = 2\alpha_i - 1
\end{equation}
Suppose we have $m$ LFs and we use majority vote algorithm on these LFs to get an estimate $\tilde{Y}$ of $Y$. The final accuracy can be given by $\mathbb{E}[Y\tilde{Y}]$ and we can get a bound on this easily using Hoeffding's inequality as following. Observe that,
$\tilde{Y} = Y$ if at most $m'=\lfloor \frac{m}{2} \rfloor-1$ LFs disagree with $Y$ since we want at least more than half of them to agree with $Y$. For simplicity we assume all LFs have same $\alpha_i=\alpha$. Let $A$ denote the number LF's in agreement with $Y$ and $D$ denote the number of LFs in disagreement with $Y$. 
\begin{equation}
	\begin{split}
		P(Y=\tilde{Y}) &= P(A\ge m') \\
		&= 1- P(A<m') \\
		&\ge 1- \exp \Big(-\frac{2m}{\alpha} \big(\alpha - \frac{m'}{m}\big)^2\Big) \\
		&\ge 1- \exp(-\frac{m(
			2\alpha - 1)^2}{2\alpha}) \qquad \qquad \frac{m'}{m} \approx \frac{1}{2}
	\end{split}      
\end{equation}
Hence,
\begin{equation}
	\begin{split}
		\mathbb{E}[Y\tilde{Y}] &= 1*P(Y=\tilde{Y}) -1*(1-P(Y=\tilde{Y}))   \\
		&= 2P(Y=\tilde{Y})-1 \\
		&\ge 1 - 2\exp(-\frac{m(
			2\alpha -1 )^2}{2\alpha})
	\end{split}
\end{equation}

Sanity Check and Interpretation:
\begin{enumerate}
	\item As we include more LFs i.e. increase $m$ the accuracy is going to increase rapidly and saturate quickly.
	\item Role of $\alpha$ is not quite clear, the quantity $\frac{(2\alpha-1)^2}{\alpha}$ decreases as $\alpha$ increases. So the exponential term is going to increase with $\alpha$ and the expected accuracy is going to decrease which is unexpected.
\end{enumerate}

\paragraph{General Case}: \\
Let $r=|S|$
\begin{equation}
	\begin{split}
		\mathbb{E}[\langle Y\pi_i \rangle] = \mathbb{E}_z[\mathbb{E}[\langle Y\pi_i\rangle |z]] &= r\alpha_i + r(2\beta_i - 1)(1-
		\alpha_i) \\
		&= r(2(\alpha_i + \beta_i - \alpha_i\beta_i) -1) 
	\end{split}
\end{equation}
So $\mathbb{E}[d_\tau(Y,\pi_i)] =2(\alpha_i + \beta_i - \alpha_i\beta_i) -1 $\\
Sanity check and interpretation:
\begin{enumerate}
	\item if $\alpha_i=1 \implies$ LF never opts to modify any ranking, $\mathbb{E}[d_\tau(Y,\pi_i)]=1$ 
	\item if $\beta_i=1 \implies$ LF never modifies any ranking even if it chooses to modify it.   $\mathbb{E}[d_\tau(Y,\pi_i)]=1$ 
	\item $\alpha_i=0 \implies \mathbb{E}[d_\tau(Y,\pi_i)]= 2\beta_i-1$, it is always choosing to modify a ranking so the correlation only depends on $\beta_i$, if $\beta_i=0$ then the correlation is -1.
	\item $\beta_i=0 \implies \mathbb{E}[d_\tau(Y,\pi_i)]= 2\alpha_i-1$, it modifies full ranking whenever it chooses to modify it. so it only depends on $\alpha_i$. 
\end{enumerate}

Suppose we follow a co-ordinate wise majority vote algorithm i.e. for $j^{th}$ coordinate (pair) we aggregate labels using majority vote algorithm and we do this for all pairs independently. We can easily get a bound on $\mathbb{E}[Y\tilde{Y}]$ for this case as following:
% \begin{equation}
%     \begin{split}
%         P(Y=\tilde{Y}) &= \prod_{j=1}^{r} P(Y^{(j)}=\tilde{Y}^{(j)}) \\
%         &\ge \Big( 1- \exp \Big( -\frac{m(2\gamma-1)^2}{2\gamma}\Big) \Big ) ^ r
%     \end{split}
% \end{equation}
\begin{equation}
	\begin{split}
		\mathbb{E}[\langle Y,\tilde{Y}\rangle] &= \sum_{j=1}^{r}\mathbb{E}[Y^{(j)}\tilde{Y}^{(j)}] \\ &\ge r -  2r\exp(-\frac{m(
			2\gamma -1 )^2}{2\gamma})
	\end{split}
\end{equation}

Here $\gamma$ is the minimum probability of agreement by a LF on a given pair with $Y$ i.e. $\gamma = \min_{i} \alpha_i + \beta_i - \alpha_i \beta_i$. We can observe that in both cases, $\mathbb{E}[d_\tau(Y,\tilde{Y})] = \frac{1}{r}\mathbb{E}[\langle Y,\tilde{Y} \rangle]\ge 1 - 2\exp \big ( -\frac{m(2\gamma-1)^2}{2\gamma}\big )$ \\
Further Questions:
\begin{itemize}
	\item How to get this bound when labels on pairs are no longer independent? Assuming independence on them is impractical for ranking setup because there exists some correlation between these pairs and one pair's label can determine the label of other pair(s). We can still treat LFs as independent.
	\item Most general and practical setup is when we don't assume independence on pairs and LFs both.(Multi task learning setup with correlation between tasks)
\end{itemize}

==> sections/learning_label_model.tex <==
\section{Learning Label Model}
\subsection{Label Model}
\subsection{Parameter Estimation}
\subsection{Inference}
  Details of aggregation rules. and theoretical results
  
  
  \begin{theorem} \cite{caragiannis2016}
  	For any given $\epsilon > 0$, any PM-c rule determines the true ranking with probability at least $1-\epsilon$ given  $\mathcal{O}(\log(\frac{d}{\epsilon}))$  samples from Mallows' model.
  \end{theorem}
  
  \begin{theorem}
  	\cite{optimalMallows2019} For any given $\pi^* \in S_d$ and $\phi^* \in [0,1-\gamma]$ Then there exist estimates $\hat{\phi}, \hat{\pi}$ which can be computed in polynomial time using $n \ge \Omega \Big( \frac{\log(1/\delta)}{d\epsilon^2} + \frac{1}{\gamma} \log(d/\delta)\Big)$ such that \begin{equation} Pr\big( (\pi^*=\hat{\pi}) \land (|\phi^*-\hat{\phi}|\le \epsilon) \big ) \ge 1-\delta.
  	\end{equation}
  \end{theorem}

\begin{theorem}
	 Weighted Kemeny Aggregation has lower sample complexity. (magnitude of weights should come in)
\end{theorem}
  
  

==> sections/macros.tex <==
\newcommand{\yell}[1]{\textcolor{red}{#1}}
% \newcommand{\assume}[1]{\textcolor{blue}{\textbf{#1}}}
\newcommand{\assume}[1]{#1}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{observation}{Observation}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{proposition}{Proposition}

%% OPERATORS:
\newcommand{\norm}[1]{\left|\left|#1\right|\right|}
\newcommand{\argmin}[2]{\textrm{argmin}_{#1}~#2}
\newcommand{\argmax}[2]{\textrm{argmax}_{#1}~#2}
% Inner product
\newcommand{\ip}[2]{\left\langle#1, #2\right\rangle}
% Trace
\newcommand{\tr}{\textrm{tr}}
% Expected value
\newcommand{\E}[2]{\mathbb{E}_{#1}\left[#2\right]}
% Sample mean
\newcommand{\Ehat}[1]{\hat{\mathbb{E}}\left[#1\right]}
% Variance
\newcommand{\Var}[2]{\textrm{Var}_{#1}\left[#2\right]}
% Covariance
\newcommand{\Cov}[2]{\textrm{\textbf{Cov}}_{#1}\left[#2\right]}
% Indicator
\newcommand{\ind}[1]{\mathbbm{1}\left\{#1\right\}}
\newcommand{\indpm}[1]{\mathbbm{1}^{\pm}\left\{#1\right\}}
% sech
\newcommand{\sech}[0]{\textrm{sech}}
% diag
\newcommand{\diagm}[1]{\textrm{diagm}\left(#1\right)}
% supp
\newcommand{\supp}{\text{supp}}
% independent
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

%\newenvironment{bsmallmatrix}
%  {\left[\begin{smallmatrix}}
%  {\end{smallmatrix}\right]}


%% VARIABLES:
% See Glossary of Symbols (Appendix A.1)
\newcommand{\x}[0]{X}
\newcommand{\p}[0]{\mathcal{P}}
\newcommand{\y}[0]{Y}
\newcommand{\lf}[0]{\lambda}
\newcommand{\lfc}[0]{\Lambda}
\newcommand{\acc}[0]{\alpha}



% LF outputs
\newcommand{\lx}[0]{\lambda}
% Observed LF outputs
\newcommand{\lfo}[0]{\bar{\lf}}
\newcommand{\lxo}[0]{\bar{\lx}}

% see line at top of main file to show/hide notes
\ifdefined\ShowNotes
  \newcommand{\colornote}[3]{{\color{#1}\bf{#2 #3}\normalfont}}
\else
  \newcommand{\colornote}[3]{}
\fi

\definecolor{darkred}{rgb}{0.7,0.1,0.1}
\definecolor{darkgreen}{rgb}{0.1,0.5,0.1}
\definecolor{cyan}{rgb}{0.7,0.0,0.7}
\definecolor{dblue}{rgb}{0.2,0.2,0.8}
\definecolor{maroon}{rgb}{0.76,.13,.28}
\definecolor{burntorange}{rgb}{0.81,.33,0}
\definecolor{royalpurple}{rgb}{0.47,.31,0.66}

\newcommand {\note}[1]{\colornote{maroon}{}{#1}}
\newcommand {\todo}[1]{\colornote{cyan}{TODO}{#1}}
\newcommand {\dan}[1]{\colornote{darkgreen}{DF:}{#1}}
\newcommand {\fred}[1]{\colornote{burntorange}{FS:}{#1}}
\newcommand {\mayee}[1]{\colornote{red}{MC:}{#1}}

% not a colornote since we don't want these to ever be removed from the document

\newcommand{\sysx}{\textsc{FlyingSquid}}
\newcommand{\avgspeedupdugong}{\num{2,300}}
\newcommand{\maxspeedupdugong}{\num{4,000}}
\newcommand{\avgspeedupdp}{\num{235}}
\newcommand{\maxspeedupdp}{\num{348}}
\newcommand{\avgspeedupdpbench}{\num{170}}
\newcommand{\maxspeedupdpbench}{\num{440}}
\newcommand{\avgspeedupdpbenchround}{\num{170}}
\newcommand{\maxspeedupdpbenchround}{\num{440}}
\newcommand{\avgslowdowndugongdp}{\num{9.5}}

\newcommand{\avglifttsall}{\num{13.4}}
\newcommand{\maxlifttsall}{\num{29.3}}
\newcommand{\avgliftmvall}{\num{14.7}}
\newcommand{\maxliftmvall}{\num{33.9}}
\newcommand{\avgliftts}{\num{12.4}}
\newcommand{\maxliftts}{\num{25.2}}
\newcommand{\avgliftmv}{\num{16.7}}
\newcommand{\maxliftmv}{\num{33.9}}
\newcommand{\avgliftdp}{\num{28.9}}
\newcommand{\maxliftdp}{\num{83.2}}
\newcommand{\avgliftdugong}{\num{1.1}}
\newcommand{\maxliftdugong}{\num{2.5}}
\newcommand{\avgliftdpbench}{\num{2.3}}
\newcommand{\maxliftdpbench}{\num{4.9}}
\newcommand{\avglifttsonline}{\num{19.8}}
\newcommand{\maxlifttsonline}{\num{36.5}}
\newcommand{\avgliftmvonline}{\num{8.9}}
\newcommand{\maxliftmvonline}{\num{15.7}}

\newcommand{\spam}{\textbf{Spam}}
\newcommand{\spouse}{\textbf{Spouse}}
\newcommand{\weather}{\textbf{Weather}}
\newcommand{\recommender}{\textbf{Recommender}}
\newcommand{\interview}{\textbf{Interview}}
\newcommand{\commercial}{\textbf{Commercial}}
\newcommand{\tennis}{\textbf{Tennis Rally}}
\newcommand{\basketball}{\textbf{Basketball}}
% \newcommand{\shot}{\textbf{Shot Detection}}


==> sections/old_notes.tex <==
\section{Old Notes}
\subsection{Known Results}
\subsubsection{Full Ranking}
\subsubsection{Single Parameter }
Its the basic setup where Mallows' distribution is parameterized by a single spread parameter $\phi \in [0,1]$ and central ranking $\pi^* \in S_d$. Here we observe $n$ i.i.d samples $\pi \in S_d$

\begin{theorem} \cite{caragiannis2016}
	For any given $\epsilon > 0$, any PM-c rule determines the true ranking with probability at least $1-\epsilon$ given  $\mathcal{O}(\log(\frac{d}{\epsilon}))$  samples from Mallows' model.
\end{theorem}

\begin{theorem}
	\cite{optimalMallows2019} For any given $\pi^* \in S_d$ and $\phi^* \in [0,1-\gamma]$ Then there exist estimates $\hat{\phi}, \hat{\pi}$ which can be computed in polynomial time using $n \ge \Omega \Big( \frac{\log(1/\delta)}{d\epsilon^2} + \frac{1}{\gamma} \log(d/\delta)\Big)$ such that \begin{equation} Pr\big( (\pi^*=\hat{\pi}) \land (|\phi^*-\hat{\phi}|\le \epsilon) \big ) \ge 1-\delta.
	\end{equation}
\end{theorem}


\textbf{RQ1} One might need samples lower than $\log(d/\epsilon)$ if the goal is to find $\hat{\pi}$ such that $d_\tau(\hat{\pi},\pi^*) \le \kappa$ 
\subsubsection{Generalized Mallows}
\cite{optimalMallows2019}

\subsection{Partial Ranking}
\subsubsection{Single Parameter}
In this setup we observe partial rankings of length $k$ over $d$ objects ($k\le d$). The The definition of Mallows' distribution is changed a bit in this case. Here $\pi^*$ is a partial ranking of length $k$ and the Kendall's Tau distance is also adapted accordingly as following, 
\begin{equation}
	d'_\tau(r1,r2) = \sum_{i,j \in r1\cup r2 \; i<j} X_{ij}
\end{equation}
\begin{equation} 
	X_{ij} = 
	\begin{cases}
		& 1 \quad \text{if } (i <_{r_1} j \text{ and } i >_{r2} j) \text{ or vice versa}  \\
		& p \quad \text{if } (i \perp_{r_1} j \text{ and } i \parallel_{r2} j) \text{ or vice versa} \\
		&  0  \quad \text{otherwise}
	\end{cases}
\end{equation}

\begin{theorem} \cite{flavioTopK2018}
	There exists a polynomial time algorithm that uses $\Theta \Big ( \frac{\phi +1}{\phi^{-1} -1} (d-k) \log d\Big  ) $ i.i.d. samples from the Mallows' distribution and can identify the central top-k list with probability $1 - o(n^{-3})$
\end{theorem}

\cite{fotakis21Selective}
\subsubsection{Generalized Mallows'}

\begin{section}{Weak Supervision with Rankings}
	\begin{itemize}
		\item Samples are from different $\phi$ but same center. We want to aggregate them to find the center. How similar is it to mixture model? Is it special case of mixture model where centers are same. Assume that $\phi$ are given, then derive sample complexity bounds to recover the center. 
		
		\item Samples are from different centers and we want to estimate $\phi$.
		
		\item Do both of the above for partial / top-k lists settings.
		
		\item Do all the above with generalized Mallows'. 
		
	\end{itemize}
\end{section}

\section{Learning accuracies of LFs in Ranking setup}
Let there be $d$ items over which $m$ LFs, give their orderings. Denote true ranking by $Y$ and ranking by $i^{th}$ LF as $\pi_i$. Let the items be indexed from $1$ to $d$ and define $S=\{(i,j): i < j ; i,j\in[d]\}$ and $S$ is ordered by $i$. In order to capture agreement and disagreement between any two rankings $r_1$ and $r_2$ we define  $\mathbf{Z}(r_1,r_2) \in \{-1,+1\}^{|
	S|}$ as following, 
\begin{equation}
	\mathbf{Z}(r_1,r_2)_i &=
	\begin{cases}
		+1 & \text{ if } r_1, r_2 \text{ agree on } i^{th} \text{ pair} \\  
		-1 & \text{ if } r_1, r_2 \text{ disagree on } i^{th} \text{ pair}
	\end{cases}
\end{equation}
Kendall Tau correlation coefficient between two rankings $r_1, r_2$ can be written as,
\begin{equation}
	d_\tau(r_1,r_2) = \frac{1}{|S|}\sum_i \mathbf{Z}(r_1,r_2)_i
\end{equation}
We want to estimate  $\mathbb{E}[ d_\tau(Y,\pi_k)]$ = $\frac{1}{|S|}\sum_{i} \mathbb{E}[ \mathbf{Z}(Y,\pi_k)_i]$ as a proxy for accuracy of $k^{th}$ LF.
Define $\mathbf{Z}^{(k)} = \mathbb{E}_{Y,\pi_k}[ \mathbf{Z}(Y,\pi_k)] \in \mathbb{R}^{|S|}$. We want to learn $\mathbf{Z}^{(k)}$ but we neither have access to the true distribution nor do we have access to samples of $Y$ so we can't even do an empirical estimation.

Observe that for any two LFs, $k,\ell$, we have  $\mathbf{Z}^{(k)}_i \cdot \mathbf{Z}^{(\ell)}_i = \mathbb{E}_{Y,\pi_k,\pi_{\ell}}[\mathbf{Z}(Y,\pi_k)_i \cdot \mathbf{Z}(Y,\pi_{\ell})_i] = \mathbb{E}_{\pi_k,\pi_{\ell}}[\mathbf{Z}(\pi_k,\pi_\ell)_i]$ . 
This holds $\mathbf{Z}(Y,\pi_k)_i \cdot \mathbf{Z}(Y,\pi_{\ell})_i = +1$ when both $\pi_k, \pi_{\ell}$ agree or disagree with $Y$ and it is equal to -1 when only one of them agrees with $Y$, which is equivalent to measuring their own agreement and disagreements.
We can have an empirical estimate $\hat{\mu}_{k,\ell}^{(i)}$ of $\mathbb{E}_{\pi_k,\pi_{\ell}}[\mathbf{Z}(\pi_k,\pi_\ell)_i]$ using which we can get empirical estimate $\hat{\mathbf{Z}}^{(j)}$ of accuracies for all LFs. 

Lets consider a simple example with three LFs. For $i^{th}$ pair,
\begin{equation}
	\begin{split}
		\hat{\mathbf{Z}}^{(1)}_i \cdot \hat{\mathbf{Z}}^{(2)}_i &=  \hat{\mu}_{1,2}^{(i)}   \\
		\hat{\mathbf{Z}}^{(2)}_i \cdot \hat{\mathbf{Z}}^{(3)}_i &=  \hat{\mu}_{2,3}^{(i)}   \\
		\hat{\mathbf{Z}}^{(1)}_i \cdot \hat{\mathbf{Z}}^{(3)}_i &=  \hat{\mu}_{1,3}^{(i)}   
	\end{split}
\end{equation}
solving this system of equation yields,
\begin{equation}
	\begin{split}
		\hat{\mathbf{Z}}^{(1)}_i &= \sqrt{\hat{\mu}_{1,2}^{(i)}\hat{\mu}_{1,3}^{(i)}/\hat{\mu}_{2,3}^{(i)}} \\
		\hat{\mathbf{Z}}^{(2)}_i &= \sqrt{\hat{\mu}_{1,2}^{(i)}\hat{\mu}_{2,3}^{(i)}/\hat{\mu}_{1,3}^{(i)}} \\
		\hat{\mathbf{Z}}^{(3)}_i &= \sqrt{\hat{\mu}_{1,3}^{(i)}\hat{\mu}_{2,3}^{(i)}/\hat{\mu}_{1,2}^{(i)}}
	\end{split}
\end{equation}
We do it for all pairs $i$ and finally get estimated accuracy of $k^{th}$ LF,  $\hat{\mathbf{Z}}^{(k)} = \frac{1}{|S|} \sum_i \hat{\mathbf{Z}}^{(k)}_i  $

\subsection{Analysis of Synthetic Setup}
Let's denote a ranking by its agreement/disagreement to a reference ranking so that each ranking belongs to $\{-1,+1\}^{|S|}$. Let $\alpha_i,\beta_i \in [0,1] $ be accuracy parameters of $i^{th}$ LF. Assume the labeling functions produce ranking by following this process:
\begin{enumerate}
	\item For given ranking $Y$, the $i^{th}$ LF will first decide whether or not make any change in $Y$ with probability $1-\alpha_i$. Denote this decision variable by $z \in \{0,1\}$, where $z=1$ indicates $Y$ will be perturbed. 
	\item If in the previous step $z=1$ then each pair in $Y$ will be inverted with probability $1-\beta_i$.
\end{enumerate}
The inner product $\langle Y,\pi_i \rangle$ tells how well do $Y,\pi_i$ agree and $\frac{1}{|S|}\langle Y,\pi_i \rangle $ is precisely the Kendall's-tau correlation coefficient between the two.
We are interested in computing $\mathbb{E}[\langle Y,\pi_i\rangle]$ which will give us the expected Kendall's tau correlation between rankings produced by LF $i$ and true rankings.
\paragraph{Binary Case}:\\

Here we have only two items i.e. a single pair hence $Y,\pi_i \in\{+1,-1\}$. In this setup $\beta_i$ doesn't make sense so we assume it be 0.
\begin{equation}
	\mathbb{E}[Y\pi_i] = (1)\alpha_i + (-1)(1-\alpha_i) = 2\alpha_i - 1
\end{equation}
Suppose we have $m$ LFs and we use majority vote algorithm on these LFs to get an estimate $\tilde{Y}$ of $Y$. The final accuracy can be given by $\mathbb{E}[Y\tilde{Y}]$ and we can get a bound on this easily using Hoeffding's inequality as following. Observe that,
$\tilde{Y} = Y$ if at most $m'=\lfloor \frac{m}{2} \rfloor-1$ LFs disagree with $Y$ since we want at least more than half of them to agree with $Y$. For simplicity we assume all LFs have same $\alpha_i=\alpha$. Let $A$ denote the number LF's in agreement with $Y$ and $D$ denote the number of LFs in disagreement with $Y$. 
\begin{equation}
	\begin{split}
		P(Y=\tilde{Y}) &= P(A\ge m') \\
		&= 1- P(A<m') \\
		&\ge 1- \exp \Big(-\frac{2m}{\alpha} \big(\alpha - \frac{m'}{m}\big)^2\Big) \\
		&\ge 1- \exp(-\frac{m(
			2\alpha - 1)^2}{2\alpha}) \qquad \qquad \frac{m'}{m} \approx \frac{1}{2}
	\end{split}      
\end{equation}
Hence,
\begin{equation}
	\begin{split}
		\mathbb{E}[Y\tilde{Y}] &= 1*P(Y=\tilde{Y}) -1*(1-P(Y=\tilde{Y}))   \\
		&= 2P(Y=\tilde{Y})-1 \\
		&\ge 1 - 2\exp(-\frac{m(
			2\alpha -1 )^2}{2\alpha})
	\end{split}
\end{equation}

Sanity Check and Interpretation:
\begin{enumerate}
	\item As we include more LFs i.e. increase $m$ the accuracy is going to increase rapidly and saturate quickly.
	\item Role of $\alpha$ is not quite clear, the quantity $\frac{(2\alpha-1)^2}{\alpha}$ decreases as $\alpha$ increases. So the exponential term is going to increase with $\alpha$ and the expected accuracy is going to decrease which is unexpected.
\end{enumerate}

\paragraph{General Case}: \\
Let $r=|S|$
\begin{equation}
	\begin{split}
		\mathbb{E}[\langle Y\pi_i \rangle] = \mathbb{E}_z[\mathbb{E}[\langle Y\pi_i\rangle |z]] &= r\alpha_i + r(2\beta_i - 1)(1-
		\alpha_i) \\
		&= r(2(\alpha_i + \beta_i - \alpha_i\beta_i) -1) 
	\end{split}
\end{equation}
So $\mathbb{E}[d_\tau(Y,\pi_i)] =2(\alpha_i + \beta_i - \alpha_i\beta_i) -1 $\\
Sanity check and interpretation:
\begin{enumerate}
	\item if $\alpha_i=1 \implies$ LF never opts to modify any ranking, $\mathbb{E}[d_\tau(Y,\pi_i)]=1$ 
	\item if $\beta_i=1 \implies$ LF never modifies any ranking even if it chooses to modify it.   $\mathbb{E}[d_\tau(Y,\pi_i)]=1$ 
	\item $\alpha_i=0 \implies \mathbb{E}[d_\tau(Y,\pi_i)]= 2\beta_i-1$, it is always choosing to modify a ranking so the correlation only depends on $\beta_i$, if $\beta_i=0$ then the correlation is -1.
	\item $\beta_i=0 \implies \mathbb{E}[d_\tau(Y,\pi_i)]= 2\alpha_i-1$, it modifies full ranking whenever it chooses to modify it. so it only depends on $\alpha_i$. 
\end{enumerate}

Suppose we follow a co-ordinate wise majority vote algorithm i.e. for $j^{th}$ coordinate (pair) we aggregate labels using majority vote algorithm and we do this for all pairs independently. We can easily get a bound on $\mathbb{E}[Y\tilde{Y}]$ for this case as following:
% \begin{equation}
%     \begin{split}
%         P(Y=\tilde{Y}) &= \prod_{j=1}^{r} P(Y^{(j)}=\tilde{Y}^{(j)}) \\
%         &\ge \Big( 1- \exp \Big( -\frac{m(2\gamma-1)^2}{2\gamma}\Big) \Big ) ^ r
%     \end{split}
% \end{equation}
\begin{equation}
	\begin{split}
		\mathbb{E}[\langle Y,\tilde{Y}\rangle] &= \sum_{j=1}^{r}\mathbb{E}[Y^{(j)}\tilde{Y}^{(j)}] \\ &\ge r -  2r\exp(-\frac{m(
			2\gamma -1 )^2}{2\gamma})
	\end{split}
\end{equation}

Here $\gamma$ is the minimum probability of agreement by a LF on a given pair with $Y$ i.e. $\gamma = \min_{i} \alpha_i + \beta_i - \alpha_i \beta_i$. We can observe that in both cases, $\mathbb{E}[d_\tau(Y,\tilde{Y})] = \frac{1}{r}\mathbb{E}[\langle Y,\tilde{Y} \rangle]\ge 1 - 2\exp \big ( -\frac{m(2\gamma-1)^2}{2\gamma}\big )$ \\
Further Questions:
\begin{itemize}
	\item How to get this bound when labels on pairs are no longer independent? Assuming independence on them is impractical for ranking setup because there exists some correlation between these pairs and one pair's label can determine the label of other pair(s). We can still treat LFs as independent.
	\item Most general and practical setup is when we don't assume independence on pairs and LFs both.(Multi task learning setup with correlation between tasks)
\end{itemize}

==> sections/theory.tex <==
%!TEX root = ../wshc-uai-draft.tex

\section{Theoretical Results}
\label{sec:theory}

\subsection{Rankings}
The Mallows model is a single-parameter model (two if you count the central permutation). It's an exponential model that penalizes permutations by distance from the central permutation $\pi^*$. The standard model looks like
\begin{align}
P_{\theta, \pi^*} = \frac{1}{Z(\theta)} \exp(-\theta d(\pi, \pi^*)),
\label{eq:mallows}
\end{align}
where $d$ is the Kendall tau distance.

A typical application is rank aggregation: get samples $\pi_1, \pi_2, \ldots, \pi_m$ from $P_{\theta, \pi^*}$ and produce an estimate of $\pi^*$, the center or mode permutation.

In our problem, we expect to have $m$ rankers, each produce a permutation $\pi$, but we know that they're not all from the same distribution. Instead, we expect them to have different accuracies; these accuracies are encoded in the parameter $\theta$ in \eqref{eq:mallows}. 

Specifically, imagine that this parameter is very large; in this case, the accuracy is quite good. If the $\theta$ instead goes to 0, then we get a uniform distribution over permutations, which means that we're completely inaccurate.

To model this, consider any distribution $\mathcal{D}$ over permutations. Then, we have the following conditional model
\begin{align}
P_{\theta_1, \theta_2, \ldots, \theta_m}(\pi_1, \pi_2, \ldots, \pi_m | \pi^*) = \frac{1}{Z} \exp(-\sum_{i=1}^m \theta_i d(\pi_i , \pi^*)),
\end{align}
where $\pi^* \sim \mathcal{D}$. One important thing to note---the $\theta_i$ accuracy parameters are not themselves a function of $\pi^*$.

Now, suppose we run the model above in the following way, We sample $\pi^* \sim \mathcal{D}$ $n$ times. Each of these times, we have a different mode permutation $\pi^*$. Then we get our $m$ values of $\pi$. We can stack these in the matrix $O$, where $O_{i,j} = \pi_i^j$ is the $i$th permutation produced by ranker $j$.

Our goal may be to learn the sequence of modes $\pi^*_1, \ldots, \pi^*_n$. Or, our goal may be to learn the accuracies $\theta_1, \ldots, \theta_m$ so that we can estimate some future mode from a single such sample. These are basically equivalent.

\paragraph{What's different} How does this differ from the standard problems above? Note that this time, while we do have $n$ samples from each marginal model with parameter $\theta_i$, these are for different permutations---so we cannot aggregate them. That is, for ranker $j$, we get to observe $O_{1}^j, O_2^j, \ldots, O_n^j$. However, these all come from different conditional models $P(\cdot | \pi^*)$, with a different $\pi^*$ for each draw, so we can't aggregate/directly learn $\theta$. Note that if all of our $\pi^*$'s are identical, we'd be back in the standard setting.

On the other hand, we do get to observe $m$ views of the same permutation $\pi^*$ for each draw from $\mathcal{D}$. But, unlike in standard rank aggregation, these do not come from the same model. Now the $\theta$ accuracy parameter is the one that changes. However, if $\theta$ is identical (same accuracy) for all $m$ rankers, we get back to the standard case.


\subsection{Continuous}

==> sections/todo.tex <==
\section{TODOs}
\subsection{Theory}
	\subsubsection{Full Ranking}
	\begin{enumerate}
		\item Write details of accuracy estimation using expected distance.
		\item How does this error $||\theta -\hat{\theta}||$ relate with final error $\mathbb{E}[ K(\pi^*,\hat{\pi})]$
		\item Get sample complexity bounds for kemeny and weighted kemeny to get $\mathbb{E}[ K(\pi^*,\hat{\pi})]\le \epsilon$
		Results from \cite{caragiannis2016,optimalMallows2019} can be used here however, in our setting we don't have samples coming from identical distributions i.e. we are aggregating samples generated with same center $\pi^*$ but different $\theta$
	\end{enumerate}
	\subsubsection{Partial Ranking}
	\begin{enumerate}
		\item Work with Top-k Mallows model from \cite{flavioTopK2018} and try same stuff as we did for full rankings.
		\item See different options for aggregation and distance notion.
	\end{enumerate}

\subsection{Experiments}
\subsubsection{Synthetic Data}
\begin{enumerate}
	\item One synthetic experiment to validate the theoretical claims for full rankings. Show parameter errors and Kendall distance between estimated centers and true centers. Emphasis is on non-homogeneous setup (LFs have varying accuracies). 
	\item One synthetic experiment to validate the theoretical claims for partial rankings. 
\end{enumerate}
\subsubsection{Real Data}
   \begin{enumerate}
   	\item Find some good applications and datasets, least 1 max 2.
   	\item Options to try out, movielens, passage-ranking for qa, 
   \end{enumerate}

\pagebreak


==> sections/triplet_proof_old.tex <==
\section{Proof of Theorems}
\begin{restatable}[]{lemma}{firstLemma}
For any $\delta>0$, two centers $y_1$ and $y_2$ with known class probabilities $p=P(Y=y_1)$, the quadratic triplet method recovers $$\alpha_i = P(g(\lambda^a)_i=1 |Y=y), \beta_i = P(g(\lambda^b)_i=1 |Y=y),..$$ for all conditionally independent label functions $\lambda_a,\lambda_b,\lambda_c$ up to error $O((\frac{\ln(2m^2/\delta)}{2n})^{1/4})$ with probability at least $1-\delta$ for all label functions if the symmetry assumption holds. 
\end{restatable}
\begin{proof}
Define \[\mu^a_i= \begin{bmatrix}P(g(\lambda^a)_i=1 |Y=y) & P(g(\lambda^a)_i=1 |Y\neq y) \\ 
P(g(\lambda^a)_i=-1 |Y=y) & P(g(\lambda^a)_i=-1 |Y\neq y)\end{bmatrix}, P = \begin{bmatrix}P(Y=y) & 0\\ 0 & P(Y\neq y)\end{bmatrix}\] and
\[O^{ab}_i = \begin{bmatrix}P(g(\lambda^a)_i=1,g(\lambda^b)_i=1) & P(g(\lambda^a)_i=1,g(\lambda^b)_i=-1) \\ P(g(\lambda^a)_i=-1,g(\lambda^b)_i=1) & P(g(\lambda^a)_i=-1,g(\lambda^b)_i=-1)\end{bmatrix}\]
By independence, we have that \begin{equation}\mu^a_iP(\mu^b_i)^T=O^{ab}_i\end{equation} Note that we can express \[P(g(\lambda^a)_i=1|Y\neq y) = \frac{P(g(\lambda^a)_i=1)}{P(Y\neq y)} - \frac{P(g(\lambda^a)_i=1|Y=y)P(Y=y)}{P(Y \neq y)}\]We can therefore rewrite the top row of $\mu_i^a$ as $[\alpha_i, c_i^a-d\alpha_i]$ where $c_i^a = \frac{P(g(\lambda^a)_i=1)}{P(Y\neq y)}$ and $d = \frac{P(Y=y)}{P(Y \neq y)}.$ After estimating the entries of $O_i$'s and $c_i$'s, we consider the top-left entry of (5) for every pair of $a,b$ and $c,$ to get the following system of equations
\begin{align}
&(1+d^2)\alpha_i\beta_i + \hat{c}_i^a\hat{c}_i^b-\hat{c}_i^ad\beta_i -\hat{c}_i^bd\alpha_i = \hat{O}_{i}^{ab}/p\\&
(1+d^2)\alpha_i\gamma_i + \hat{c}_i^a\hat{c}_i^c-\hat{c}_i^ad\gamma_i -\hat{c}_i^cd\alpha_i =\hat{O}_{i}^{ac}/p \\&
(1+d^2)\beta_i\gamma_i + \hat{c}_i^b\hat{c}_i^c-\hat{c}_i^bd\gamma_i -\hat{c}_i^cd\beta_i =\hat{O}_{i}^{bc}/p
\end{align} where $\beta_i$ and $\gamma_i$ are the top-left entries of $\mu_i^b$ and $\mu_i^c$ respectively.
Dropping the $i$ subscript for ease of notation and rearranging the first and third equations gives us expressions for $\alpha$ and $\gamma$ in terms of $\beta.$ 
\begin{align*}
\alpha = \frac{\hat{O}_{ab}/p+\hat{c}_ad\beta-\hat{c}_a\hat{c}_b}{(1+d^2)\beta -\hat{c}_bd} \\
\gamma = \frac{\hat{O}_{bc}/p+\hat{c}_cd\beta-\hat{c}_b\hat{c}_c}{(1+d^2)\beta -\hat{c}_bd}
\end{align*}
Substituting into (7)  gives
\begin{multline*}(1+d^2) \frac{\hat{c}_ad\beta + \hat{O}_{ab}/p-\hat{c}_a\hat{c}_b}{(1+d^2)\beta -\hat{c}_bd}\cdot \frac{\hat{c}_cd\beta + \hat{O}_{bc}/p-\hat{c}_b\hat{c}_c}{(1+d^2)\beta -\hat{c}_bd} + \hat{c}_a\hat{c}_c \\ -\hat{c}_ad \frac{\hat{c}_cd\beta + \hat{O}_{bc}/p-\hat{c}_b\hat{c}_c}{(1+d^2)\beta -\hat{c}_bd} -\hat{c}_cd\frac{\hat{c}_ad\beta + \hat{O}_{ab}/p-\hat{c}_a\hat{c}_b}{(1+d^2)\beta -\hat{c}_bd} = \hat{O}_{ac}/p \end{multline*}
We can multiply the equation by $((1+d^2)\beta -\hat{c}_bd)^2$ to get
\begin{gather*}
(1+d^2)(\hat{c}_ad\beta + \hat{O}_{ab}/p-\hat{c}_a\hat{c}_b)\cdot (\hat{c}_cd\beta + \hat{O}_{bc}/p-\hat{c}_b\hat{c}_c) + \hat{c}_a\hat{c}_c(((1+d^2)\beta -\hat{c}_bd)^2)\\ -\hat{c}_ad(\hat{c}_cd\beta + \hat{O}_{bc}/p-\hat{c}_b\hat{c}_c)\cdot ((1+d^2)\beta -\hat{c}_bd) - \hat{c}_cd(\hat{c}_ad\beta + \hat{O}_{ab}/p-\hat{c}_a\hat{c}_b)\cdot((1+d^2)\beta -\hat{c}_bd) \\
= \hat{O}_{ac}/p\cdot ((1+d^2)\beta -\hat{c}_bd)^2 
\end{gather*}
\begin{gather*}
\Rightarrow (1+d^2)\bigg(\hat{c}_a\hat{c}_cd^2\beta^2 + (\hat{O}_{ab}/p-\hat{c}_a\hat{c}_b)\hat{c}_cd\beta + (\hat{O}_{bc}/p-\hat{c}_b\hat{c}_c)\hat{c}_ad\beta + (\hat{O}_{ab}/p-\hat{c}_a\hat{c}_b)(\hat{O}_{bc}/p-\hat{c}_b\hat{c}_c)\bigg) \\ 
+ \hat{c}_a\hat{c}_c\bigg( (1+d^2)(1+d^2)\beta^2  - \hat{c}_bd(1+d^2)\beta - \hat{c}_bd(1+d^2)\beta +\hat{c}_b^2d^2 \bigg) \\ 
- \hat{c}_ad \bigg( \hat{c}_cd(1+d^2)\beta^2 + (\hat{O}_{bc}/p-\hat{c}_b\hat{c}_c)(1+d^2)\beta - \hat{c}_b\hat{c}_cd^2\beta -\hat{c}_bd(\hat{O}_{bc}/p-\hat{c}_b\hat{c}_c) \bigg) \\ 
- \hat{c}_cd\bigg( \hat{c}_ad(1+d^2)\beta^2 + (\hat{O}_{ab}/p-\hat{c}_a\hat{c}_b)(1+d^2)\beta - \hat{c}_a\hat{c}_bd^2\beta -\hat{c}_bd(\hat{O}_{ab}/p-\hat{c}_a\hat{c}_b) \bigg) \\ = \hat{O}_{ac}/p\cdot \bigg( (1+d^2)(1+d^2)\beta^2  -2\hat{c}_bd(1+d^2)\beta +\hat{c}_b^2d^2 \bigg)
\end{gather*}
\begin{gather*}
\Rightarrow \beta^2 \bigg[ (1+d^2)\hat{c}_a\hat{c}_cd^2 + \hat{c}_a\hat{c}_c(1+d^2)(1+d^2) - \hat{c}_a\hat{c}_cd^2(1+d^2)\\ - \hat{c}_a\hat{c}_cd^2(1+d^2) -\hat{O}_{ac}/p\cdot (1+d^2)(1+d^2) \bigg] \\
 + \beta \bigg[ (1+d^2)\bigg((\hat{O}_{ab}/p-\hat{c}_a\hat{c}_b)\hat{c}_bd + (\hat{O}_{bc}/p-\hat{c}_b\hat{c}_c)\hat{c}_ad\bigg) + \hat{c}_a\hat{c}_c\bigg( -\hat{c}_bd(1+d^2)-\hat{c}_bd(1+d^2) \bigg)\\ - \hat{c}_ad\bigg( (\hat{O}_{bc}/p-\hat{c}_b\hat{c}_c)(1+d^2)-\hat{c}_b\hat{c}_cd^2\bigg) - \hat{c}_cd \bigg( (\hat{O}_{ab}/p-\hat{c}_a\hat{c}_b)(1+d^2) -\hat{c}_a\hat{c}_bd^2\bigg) \\+ \hat{O}_{ac}/p \cdot \bigg( 2\hat{c}_bd(1+d^2) \bigg)\bigg] \\ + \bigg[ (1+d^2)(\hat{O}_{ab}/p-\hat{c}_a\hat{c}_b)(\hat{O}_{bc}/p-\hat{c}_b\hat{c}_c)  + \hat{c}_a\hat{c}_c\hat{c}_b^2d^2 \\ +\hat{c}_a\hat{c}_bd^2(\hat{O}_{bc}/p-\hat{c}_b\hat{c}_c) + \hat{c}_b\hat{c}_cd^2(\hat{O}_{ab}/p-\hat{c}_a\hat{c}_b) - \hat{O}_{ac}/p\cdot \hat{c}_b^2d^2\bigg] = 0
\end{gather*}
The only sources of error are from estimating $c$'s and $O$'s.Let $\epsilon_{c'}$ denote the error for the $c$'s. Let $\epsilon_O$ denote the error from $O$'s. The quadratic formula is $\beta = \frac{-b\pm \sqrt{b^2-4ac}}{2a}$ where 
\[
a = (1+d^2)\hat{c}_a\hat{c}_cd^2 + \hat{c}_a\hat{c}_c(1+d^2)(1+d^2) -  2\hat{c}_a\hat{c}_cd^2(1+d^2) -\hat{O}_{ac}/p\cdot (1+d^2)(1+d^2) \]
\begin{gather*}
b=   (1+d^2)\bigg((\hat{O}_{ab}/p-\hat{c}_a\hat{c}_b)\hat{c}_bd + (\hat{O}_{bc}/p-\hat{c}_b\hat{c}_c)\hat{c}_ad\bigg) + \hat{c}_a\hat{c}_c\bigg( -2\hat{c}_bd(1+d^2) \bigg)\\ - \hat{c}_ad\bigg( (\hat{O}_{bc}/p-\hat{c}_b\hat{c}_c)(1+d^2)-\hat{c}_b\hat{c}_cd^2\bigg) - \hat{c}_cd \bigg( (\hat{O}_{ab}/p-\hat{c}_a\hat{c}_b)(1+d^2) -\hat{c}_a\hat{c}_bd^2\bigg) \\+ \hat{O}_{ac}/p \cdot \bigg( 2\hat{c}_bd(1+d^2)  \bigg)\end{gather*} 
\begin{gather*}c=  (1+d^2)(\hat{O}_{ab}/p-\hat{c}_a\hat{c}_b)(\hat{O}_{bc}/p-\hat{c}_b\hat{c}_c)  + \hat{c}_a\hat{c}_c\hat{c}_b^2d^2  +\hat{c}_a\hat{c}_bd^2(\hat{O}_{bc}/p-\hat{c}_b\hat{c}_c) \\+ \hat{c}_b\hat{c}_cd^2(\hat{O}_{ab}/p-\hat{c}_a\hat{c}_b) - \hat{O}_{ac}/p\cdot \hat{c}_b^2d^2
\end{gather*}

Let $\epsilon_a,\epsilon_b,\epsilon_c$ denote the error from each term. Then 
\[
\epsilon_a = O\left(\frac{(1+d^2)d^2}{1-p}\epsilon_{c'}+\frac{(1+d^2)^2}{p}\cdot\epsilon_O\right)\]
\[\epsilon_b = O\left(d(1+d^2)\left(\frac{\epsilon_O}{p(1-p)}+\frac{\epsilon_{c'}}{p}\right)\right)\]
\[\epsilon_c = O\left((1+d^2) \left(\frac{\epsilon_O}{p^3}+\frac{\epsilon_{c'}}{p^3}\right)\right)\]
Because $d$ is defined with respect to $p,$ if we ignore the dependence on $p,$ we get that 
\[\epsilon_a=\epsilon_b=\epsilon_c = O(\epsilon_{c'}+\epsilon_O)\]
Furthermore, \[\epsilon_{b^2}=O(\epsilon_b), \epsilon_{ac}=O(\epsilon_a+\epsilon_c)\] It follows that \[\epsilon_\beta =O\bigg( \frac{\epsilon_b+\sqrt{\epsilon_a+\epsilon_b+\epsilon_c}}{2a-\epsilon_a}\bigg)+O\bigg(\frac{(-b\pm\sqrt{b^2-4ac})\epsilon_a}{a(a-\epsilon_a)}\bigg)\]
\[= O(\sqrt{\epsilon_{c'}+\epsilon_O})\] Since $O$ and $c$ are Bernoulli random variables, by Hoeffding's inequality and union bound, with probability at least $1-\frac{\delta}{2},$ $\epsilon_{c_i} \leq \sqrt{\frac{\ln(2m/\delta)}{2n}}$ for all $i \in [m],$ and with probability at least $1-\frac{\delta}{2},$ $\epsilon_{O_{ij}} \leq \sqrt{\frac{\ln(2 \binom{m}{2}/\delta)}{2n}}$ for all $i,j \in [m].$ It follows that with probability at least $1-\delta,$ $\epsilon_\alpha = \epsilon_\gamma = ... = O((\frac{\ln(2m^2/\delta)}{2n})^{1/4}).$ 
\end{proof} 
We can now prove the main theorem in the rankings case.  \estimateTheta*

\begin{proof} Consider a pair of items $(a,b).$ Without loss of generality, suppose $a\prec_{y_1}b$ and $a\succ_{y_2}b.$ Define $\alpha_{a,b} = P(a\prec_{\lambda^a}b|y_1),$ $\alpha'_{a,b} = P(a\succ_{\lambda^a}b|y_2)$ then our estimate for $P(\lambda^a_{(a,b)} \sim Y_{(a,b)})$ where $\lambda^a_{(a,b)} \sim Y_{(a,b)}$ denotes the event that label function $i$ ranks $(a,b)$ correctly would be \[\hat{P}(\lambda^a_{(a,b)}\sim Y_{(a,b)})= p\hat{\alpha}_{a,b} + (1-p)(1-\hat{\alpha'}_{a,b})\] which has error $O(\epsilon_\alpha).$ Then, note that $E[d(\lambda^a,Y)] = \sum_{a,b}P(\lambda^a_{(a,b)}\sim Y_{(a,b)}).$ Therefore, we can compute the estimate $\hat{E}[d(\lambda^a,Y)] = \sum_{a,b} \hat{E}[\lambda_i\sim Y]_{a,b}$ which has error $ O(\binom{\rho}{2}(\frac{\ln(6)/\delta}{2n})^{1/4})$.\newline \newline It is a fact (Fligner and Verducci) that \[E_\theta[D] = \frac{d[\log(M(t))]}{dt}\bigg|_{t=-\theta}\] where $M(t)$ is the moment generating function, which can be shown to satisfy (Chierichetti et al.)
\[M(t) = \frac{1}{k!}\prod_{j\leq k}\frac{1-e^{\theta j}}{1-e^\theta}.\] It follows that \begin{equation}E_\theta[D]= \frac{ke^{-\theta}}{1-e^{-\theta}}-\sum_{j\leq k}\frac{je^{-\theta j}}{1-e^{-\theta j}}\end{equation} \[\Rightarrow \frac{d}{d\theta}E_\theta[D] = \frac{-ke^{-\theta}}{(1-e^{-\theta})^2} + \sum_{j\leq k} \frac{j^2e^{-\theta j}}{(1-e^{-\theta j})^2}\] Let $g_k(\theta) = \frac{-ke^{-\theta}}{(1-e^{-\theta})^2}+\sum_{j\leq k} \frac{j^2e^{-\theta j}}{(1-e^{-\theta j})^2}.$ By Lemma 0.3, $g_k$ is non positive and increasing in $\theta$ for $\theta >0$. It follows that by numerically computing the inverse function of (9), our estimate of $\theta$ has error $O(\frac{\rho^2}{|g_2(U)|}(\frac{\ln(2m^2)/\delta}{2n})^{1/4}).$  \end{proof}
\begin{lemma}
$g_k$ is non-positive and increasing in $\theta$ for  $\theta > 4\ln(2).$ Additionally, $g_k$ is decreasing in $k.$
\end{lemma}
\begin{proof}
We first show non-positivity. For this, it is sufficient to show 
\begin{equation}\frac{j^2e^{-\theta j}}{(1-e^{-\theta j})^2} \leq \frac{e^{-\theta}}{(1-e^{-\theta})^2}\end{equation} holds for all $1\leq j $ and $\theta>0.$ This clearly holds for $j=1.$
Rearranging gives
\[j^2e^{-\theta(j-1)} \leq \bigg(\frac{1-e^{-\theta j}}{1-e^{-\theta}}\bigg)^2\]
The right-hand term is greater than or equal to 1, so it suffices to choose $\theta$ such that
\[j^2e^{-\theta(j-1)}\leq 1\]
\[\Rightarrow \theta \geq \frac{\ln(j^2)}{j-1}\] It can be shown that the right-hand term decreases with $j$ for $j>1,$ so it suffices to take $j =2,$ which implies $\theta \geq 2\ln(2).$ By choice of $\theta$ this is clearly true. \newline \newline
To show that $g_k$ is increasing in $\theta,$ we consider \[\frac{d}{d\theta}g_k(\theta) = \frac{ke^{-\theta}(1-e^{-2\theta})}{(1-e^{-\theta})^4} + \sum_{j \leq k}\frac{j^3e^{-\theta j}(e^{-2\theta j}-1)}{(1-e^{-\theta j})^4}\] Similarly, it suffices to show \[\frac{j^3e^{-\theta j}(1-e^{-2\theta j})}{(1-e^{-\theta j})^4} \leq \frac{e^{-\theta}(1-e^{-2\theta})}{(1-e^{-\theta})^4}\] Rearranging, we have
\[j^3e^{-\theta (j-1)} \leq \frac{1-e^{-2\theta}}{1-e^{-2\theta j}}\bigg(\frac{1-e^{-\theta j}}{1-e^{-\theta}}\bigg)^4\] Note that
\[\frac{1-e^{-2\theta}}{1-e^{-2\theta j}}\bigg(\frac{1-e^{-\theta j}}{1-e^{-\theta}}\bigg)^4 \geq \frac{1-e^{-\theta j}}{1-e^{-2\theta j}}\] The term on the right is greater than $\frac{1}{2}$ for $\theta >0$ and $j\geq 1.$ Therefore, it suffices to choose $\theta$ such that
\[j^3e^{-\theta(j-1)}\leq \frac{1}{2}\]
\[\Rightarrow \theta \geq \frac{\ln(2j^3)}{j-1}\] Once again, the term on the right is decreasing in $j,$ so we can take $j=2,$ giving $\theta \geq 4\ln(2),$ which is satisfied by our choice of $\theta.$ \newline \newline
Finally, the fact that $g_k$ is decreasing in $k$ follows from (4).
\end{proof}


\estimateA*

\begin{proof}
For three conditionally independent label functions $\lambda_a,\lambda_b,\lambda_c$, our estimate of $a_a$ is 
\begin{align*}
|\hat{a}_{a}| = \left(\frac{|\hat{e}_{ab}| |\hat{e}_{a,c}|E[Y^2]}{|\hat{e}_{b,c}|}\right)^{\frac{1}{2}}
\end{align*}

Furthermore, if we define $x_{a,b} = \frac{|\hat{e}_{a,b}|}{|e_{a,b}|}$, we can write the ratio of elements of $\hat{a}$ to $a$ as 
\begin{align*}
k_{i} = \frac{|\hat{a}_{i}|}{|a_{i}|} = \left(\frac{|\hat{e}_{i j}|}{|e_{i j}|} \cdot \frac{|\hat{e}_{a,c}|}{|e_{a,c}|} \cdot \frac{|e_{b,c}|}{|\hat{e}_{b,c}|} \right)^{\frac{1}{2}} = \left(\frac{x_{i j} x_{a,c}}{x_{b,c}} \right)^{\frac{1}{2}}
\end{align*}

(and definitions would be symmetric for $k_{j}$ and $k_{k}$). Now note that because we assume that signs are completely recoverable, 
$
||\hat{a}_a - a_a||_2 = | |\hat{a}_a| - |a_a| |_2
$.

Note that $|\hat{a}_a^2 - a_a^2| = |\hat{a}_a - a_a| |\hat{a}_a + a_a |$. By the reverse triangle inequality, $(|\hat{a}_a| - |a_a|)^2 = ||\hat{a}_a| - |a_a||^2 \le |\hat{a}_a - a_a|^2 = \left( \frac{|\hat{a}_a^2 - a_a^2 |}{|\hat{a}_a + a_a|}\right)^2 \le \frac{1}{c^2} |\hat{a}^2_a - a^2_a|^2$, where we define $c$ as $\min_a |\hat{a}_a + a_a|$. (With high probability $c = \hat{a}_{|min|}| + |a_{|min|}$, but there is a chance that $\hat{a}_a$ and $a_a$ have opposite signs.) For ease of notation, suppose we examine a particular $(a,b,c) = (1, 2, 3)$. Then
\begin{align*}
(|\hat{a}_1| - |a_1|)^2 &\le \frac{1}{c^2}|\hat{a}_1^2 - a_1^2|^2 = \frac{1}{c^2} \Bigg| \frac{|\hat{e}_{12}| |\hat{e}_{13}|}{|\hat{e}_{23}|} - \frac{|e_{12}| |e_{13}|}{|e_{23}|} \Bigg|^2 \\
&= \frac{1}{c^2} \Bigg| \frac{|\hat{e}_{12}| |\hat{e}_{13}|}{|\hat{e}_{23}|} - \frac{|\hat{e}_{12}| |\hat{e}_{13}|}{|e_{23}|} + \frac{|\hat{e}_{12}| |\hat{e}_{13}|}{|e_{23}|} - \frac{|\hat{e}_{12}| |e_{13}|}{|e_{23}|} +  \frac{|\hat{e}_{12}| |e_{13}|}{|e_{23}|} - \frac{|e_{12}| |e_{13}|}{|e_{23}|} \Bigg|^2 \\
&\le\frac{1}{c^2} \left(\Big|\frac{\hat{e}_{12} \hat{e}_{13}}{\hat{e}_{23} e_{23}}\Big| ||\hat{e}_{23}| - |e_{23}| | + \Big|\frac{\hat{e}_{12}}{e_{23}} \Big| ||\hat{e}_{13}| - |e_{13}|| + \Big|\frac{e_{13}}{e_{23}} \Big| ||\hat{e}_{12}| - |e_{12}||\right)^2 \\
&\le \frac{1}{c^2} \left(\Big|\frac{\hat{e}_{12} \hat{e}_{13}}{\hat{e}_{23} e_{23}}\Big| |\hat{e}_{23} - e_{23}| + \Big|\frac{\hat{e}_{12}}{e_{23}} \Big| |\hat{e}_{13} - e_{13}| + \Big|\frac{e_{13}}{e_{23}} \Big| |\hat{e}_{12} - e_{12}|\right)^2
\end{align*}

With high probability, all elements of $\hat{e}$ and $e$ must be less than $e_{max}=\max_{j,k}e_{j,k}$. We further know that elements of $|e|$ are at least $a_{|min|}^2/E[Y^2]$. Now suppose (with high probability) that elements of $|\hat{e}|$ are at least $\hat{a}_{|min|}^2 > 0$, and define $\triangle_{a,b} = \hat{e}_{a,b} - e_{a,b}$. Then
\begin{align*}
(|\hat{a}_1| - |a_1|)^2 &\le \frac{\max(e_{max},e_{max}^2)}{c^2} \left(\frac{1}{a_{|min|}^2 \hat{a}_{|min|}^2E[Y^2]^2} |\triangle_{23}| + \frac{1}{a_{|min|}^2E[Y^2]} |\triangle_{13}| + \frac{1}{a_{|min|}^2E[Y^2]} |\triangle_{12}|\right)^2 \\
&\le \frac{\max(e_{max},e_{max}^2)}{c^2}(\triangle_{23}^2 + \triangle_{13}^2 + \triangle_{12}^2)\left(\frac{1}{a^4_{|min|} \hat{a}^4_{|min|}E[Y^2]^4} + \frac{2}{a^4_{|min|}E[Y^2]^2}\right)
\end{align*}

The original expression is now
\begin{align*}
||\hat{a}_a - a_a||_2 \le \left( \frac{\max(e_{max},e_{max}^2)}{c^2}\left(\frac{1}{a_{|min|}^4 \hat{a}_{|min|}^4E[Y^2]^4} + \frac{2}{a_{|min|}^4E[Y^2]^2} \right)(\triangle_{a,b}^2 + \triangle_{a,c}^2 + \triangle_{b,c}^2) \right)^{\frac{1}{2}}
\end{align*}

To bound the maximum absolute value between elements of $\hat{e}$ and $e$, note that 
\begin{align*}
\left(2\left(\triangle^2_{i j} + \triangle^2_{a,c} + \triangle^2_{b,c}\right) \right)^{\frac{1}{2}} \leq ||\hat{e}_{a,b,c} - e_{a,b,c}||_F 
\end{align*}
Where $e_{a,b,c}$ is a 3 $\times$ 3 matrix with $e_{i,j}$ in the $(i,j)$-th position.  
Moreover, it is a fact that $||\hat{e}_{a,b,c} - e_{a,b,c}||_F \leq \sqrt{r} ||\hat{e}_{a,b,c} - e_{a,b,c} ||_2 \le \sqrt{3} ||\hat{e}_{a,b,c} - e_{a,b,c} ||_2$ where $r$ is the rank of $\hat{e}_{a,b,c} - e_{a,b,c}$. Putting everything together,

\begin{align*}
|| \hat{a}_a - a_a||_2 &\le \left( \frac{\max(e_{max},e_{max}^2)}{c^2}\left(\frac{1}{a_{|min|}^4 \hat{a}_{|min|}^4E[Y^2]^4} + \frac{2}{a_{|min|}^4E[Y^2]^2} \right) \cdot \frac{1}{2} ||\hat{e}_{a,b,c} - e_{a,b,c} ||_F^2 \right)^{\frac{1}{2}} \\
&\le \left( \frac{\max(e_{max},e_{max}^2)}{c^2}\left(\frac{1}{a_{|min|}^4 \hat{a}_{|min|}^4E[Y^2]^4} + \frac{2}{a_{|min|}^4E[Y^2]^2} \right) \cdot \frac{3}{2} ||\hat{e}_{a,b,c} - e_{a,b,c} ||_2^2 \right)^{\frac{1}{2}}
\end{align*}

Lastly, to compute $\mathbb{E}[||\hat{a}_a - a_a||_2]$, we use Jensen's inequality (concave version, due to the square root) and linearity of expectation:
\begin{align*}
\mathbb{E}|| \hat{a} - a||_2] \le \left( \frac{\max(e_{max},e_{max}^2)}{c^2}\left(\frac{1}{a_{|min|}^4 \hat{a}_{|min|}^4E[Y^2]^4} + \frac{2}{a_{|min|}^4E[Y^2]^2} \right) \cdot \frac{3}{2}  \mathbb{E}[||\hat{e}_{a,b,c} - e_{a,b,c} ||_2^2] \right)^{\frac{1}{2}}
\end{align*}

We use the covariance matrix inequality as described in \cite{eetal}, which says
\begin{align*}
P(||\hat{e} - e||_2 \ge \gamma) \le \max\left(2e^{3-\frac{n\gamma}{\sigma^2C}},2e^{3-\frac{n\gamma^2}{\sigma^4C^2}}\right)
\end{align*} where $\sigma = \max_a e_{aa}$ and $C>0$ is a universal constant.

To get the probability distribution over $||\hat{e} - e||_2^2$, we just note that $P(||\hat{e} - e||_2 \ge \gamma) = P(||\hat{e} - e||_2^2 \ge \gamma^2)$ to get
\begin{align*}
P(||\hat{e} - e||_2^2 \ge \gamma) \le 2e^3\max\left(e^{-\frac{n\sqrt{\gamma}}{\sigma^2C}},e^{-\frac{n\gamma}{\sigma^4C^2}}\right)
\end{align*}

From which we can integrate to get
\begin{align*}
\mathbb{E}[||\hat{e}_{a,b,c} - e_{a,b,c}||^2_2 ] = \int_0^{\infty} P(||\hat{e_{a,b,c}} - e_{a,b,c}||_2^2 \ge \gamma) d\gamma \le 2e^3\max\left(\frac{\sigma^4C^2}{n},2\frac{\sigma^4C^2}{n^2}\right) = O(\frac{\sigma^4}{n})
\end{align*}

Substituting this back in, we get
\begin{align*}
\mathbb{E}[|| \hat{a} - a||_2] &\le \left( \frac{\max(e_{max},e_{max}^2)}{(\hat{a}_{|min|} + a_{|min|})^2}\left(\frac{1}{a_{|min|}^4 \hat{a}_{|min|}^4E[Y^2]^4} + \frac{2}{a_{|min|}^4E[Y^2]^2} \right) \cdot  O\left(\frac{\sigma^4}{n}\right) \right)^{\frac{1}{2}} \\
&\le \left( \frac{\max(e_{max},e_{max}^2)}{(\hat{a}_{|min|} + a_{|min|})^2} \cdot \left(\frac{1}{a_{|min|}^4 \hat{a}_{|min|}^4E[Y^2]^4} + \frac{2}{a_{|min|}^4E[Y^2]^2} \right) \cdot O\left(\frac{\sigma^4}{n}\right)\right)^{\frac{1}{2}}\\&
\le \left( \frac{\max(e_{max},e_{max}^2)}{(\hat{a}_{|min|} + a_{|min|})^2\min(E[Y^2]^4,E[Y^2]^2)} \cdot \left(\frac{1}{a_{|min|}^4 \hat{a}_{|min|}^4} + \frac{2}{a_{|min|}^4} \right) \cdot O\left(\frac{\sigma^4}{n}\right)\right)^{\frac{1}{2}}
\end{align*}


with high probability. Finally, we try to clean up the $a_{|min|}$ and $\hat{a}_{|min|}$ terms. The terms involving $a$ and $\hat{a}$ can be rewritten as
\begin{align*}
\frac{1 + 2\hat{a}^4_{|min|}}{a^6_{|min|} \hat{a}^4_{|min|} + 2a_{|min|}^5 \hat{a}_{|min|}^5 + a^4_{|min|} \hat{a}^6_{|min|}} 
\end{align*}

We suppose that $\frac{\hat{a}_{|min|}}{a_{|min|}} \in [1 - \epsilon, 1 + \epsilon]$ for some $\epsilon > 0$ with high probability. Then, this becomes less than
\begin{align*}
\frac{1 + 2\hat{a}^4_{|min|}}{(1 - \epsilon)^4 a^{10}_{|min|} + 2(1 - \epsilon)^5 a^{10}_{|min|} + (1 - \epsilon)^6 a^{10}_{|min|}} &\le \frac{1 + 2\hat{a}^4_{|min|}}{4(1 - \epsilon)^6 a^{10}_{|min|}} \\& 
= O\left(\frac{1}{a^{10}_{|min|}}+ \frac{1}{a^{6}_{|min|}}\right)
\end{align*}

Therefore, with high probability, the sampling error for the accuracy is bounded by
\[
\mathbb{E}[||\hat{a}_a - a_a||_2] = O\left( \sigma^2\left(\frac{1}{a^{10}_{|min|}}+ \frac{1}{a^{6}_{|min|}}\right) \sqrt{\frac{\max(e_{max},e_{max}^2)}{n}}\right)
\]

\end{proof}


==> todos.tex <==
\section{TODOs}
\begin{itemize}
    \item Review section 2, 3 (notations, formulations)
    \item Check consistency between section 4 and appendix D, E.
    \item Improve appendix D - too short explanations such as ``Next, we note that it is possible to show that the sample complexity of learning the permutationy using thisestimator is still $\Theta(log(m/\delta))$ by using the pairwise majority result in Caragiannis et al. (2016)."
    \item Add more related works regarding riemannian manifold and generic metric space learning
    \item Review appendix F - especially formulations.
\end{itemize}
\pagebreak

